Axial charges of hyperons and charmed baryons using $N_f=2+1+1$ twisted mass fermions

The axial couplings of the low lying baryons are evaluated using a total of five ensembles of dynamical twisted mass fermion gauge configurations. The simulations are performed using the Iwasaki gauge action and two degenerate flavors of light quarks, and a strange and a charm quark fixed to approximately their physical values at two values of the coupling constant. The lattice spacings, determined using the nucleon mass, are $a=0.082$ fm and $a=0.065$ fm and the simulations cover a pion mass in the range of about 210 MeV to 430 MeV. We study the dependence of the axial couplings on the pion mass in the range of about 210 MeV to 430 MeV as well as the $SU(3)$ breaking effects as we decrease the light quark mass towards its physical value.

==> tables/table_B25.tex <==
 $ N                 $     &   -0.2587(345)       &   0.7797(527)                 &   -                 &   -       &   1.1089(467)       &   0.5376(485)       &   0.5376(485)       &   0.5376(485)     \\ 
 $\Lambda            $      &   0.0248(169)      &   -0.1148(142)       &   0.7264(112)                 &   -       &   0.1399(237)      &   -1.5439(278)       &   0.6352(247)       &   0.6352(247)     \\ 
 $\Sigma^+           $      &   0.8141(468)                 &   -      &   -0.2751(210)                 &   -       &   0.8141(468)       &   1.3630(591)       &   0.5374(536)       &   0.5374(536)     \\ 
 $\Sigma^0           $      &   0.4597(224)       &   0.3187(175)      &   -0.2628(144)                 &   -       &   0.1392(265)       &   1.3040(463)       &   0.5152(304)       &   0.5152(304)     \\ 
 $\Sigma^-           $                &   -       &   0.7565(379)      &   -0.2735(149)                 &   -      &   -0.7565(379)       &   1.3029(534)       &   0.4875(370)       &   0.4875(370)     \\ 
 $\Xi^0              $     &   -0.2495(159)                 &   -       &   0.9198(205)                 &   -      &   -0.2495(159)      &   -2.0903(448)       &   0.6742(235)       &   0.6742(235)     \\ 
 $\Xi^-              $                &   -      &   -0.2712(117)       &   0.9308(155)                 &   -       &   0.2712(117)      &   -2.1412(270)       &   0.6320(326)       &   0.6320(326)     \\ 
 $\Delta^{++}        $     &   1.7171(1326)                 &   -                 &   -                 &   -      &   1.7171(1326)      &   1.7171(1326)      &   1.7171(1326)      &   1.7171(1326)     \\ 
 $\Delta^{+}         $     &   1.1264(1213)       &   0.5688(767)                 &   -                 &   -      &   0.5681(1481)      &   1.6891(1391)      &   1.6891(1391)      &   1.6891(1391)     \\ 
 $\Delta^{0}         $      &   0.4992(640)      &   1.0905(1061)                 &   -                 &   -     &   -0.5940(1170)      &   1.5903(1294)      &   1.5903(1294)      &   1.5903(1294)     \\ 
 $\Delta^{-}         $                &   -      &   1.7354(1721)                 &   -                 &   -     &   -1.7354(1721)      &   1.7354(1721)      &   1.7354(1721)      &   1.7354(1721)     \\ 
 $\Sigma^{*+}        $      &   1.1483(722)                 &   -       &   0.6534(268)                 &   -       &   1.1483(722)      &   -0.1560(630)       &   1.8010(893)       &   1.8010(893)     \\ 
 $\Sigma^{*0}        $      &   0.5590(355)       &   0.5461(421)       &   0.6535(225)                 &   -       &   0.0148(543)      &   -0.1985(529)       &   1.7568(692)       &   1.7568(692)     \\ 
 $\Sigma^{*-}        $                &   -       &   1.0665(663)       &   0.6430(252)                 &   -      &   -1.0665(663)      &   -0.2122(664)       &   1.7121(792)       &   1.7121(792)     \\ 
 $\Xi^{*0}           $      &   0.5796(279)                 &   -       &   1.3089(344)                 &   -       &   0.5796(279)      &   -2.0378(618)       &   1.8884(531)       &   1.8884(531)     \\ 
 $\Xi^{*-}           $                &   -       &   0.5434(304)       &   1.2827(307)                 &   -      &   -0.5434(304)      &   -2.0217(603)       &   1.8263(491)       &   1.8263(491)     \\ 
 $\Omega^-           $                &   -                 &   -       &   1.9642(377)                 &   -                 &   -      &   -3.9284(753)       &   1.9642(377)       &   1.9642(377)     \\ 
 $\Lambda_c^+        $       &   0.0049(83)       &   -0.0276(80)                 &   -        &   0.9157(94)       &   0.0331(116)      &   -0.0222(115)      &   -2.7833(245)       &   0.8886(187)     \\ 
 $\Xi_c^+            $      &   -0.0149(54)                 &   -       &   -0.0056(43)        &   0.9196(78)       &   -0.0149(54)       &   -0.0040(80)      &   -2.7903(226)       &   0.8613(312)     \\ 
 $\Xi_c^0            $                &   -       &   -0.0255(45)        &   0.0029(42)       &   0.8813(174)        &   0.0255(45)        &   0.0255(45)      &   -2.7885(175)       &   0.7441(632)     \\ 
 $\Sigma_c^{++}      $      &   0.7907(306)                 &   -                 &   -      &   -0.3253(196)       &   0.7907(306)       &   0.7907(306)       &   1.7630(722)       &   0.4653(322)     \\ 
 $\Sigma_c^{+}       $      &   0.3933(190)       &   0.3505(182)                 &   -      &   -0.3268(178)       &   0.0405(236)       &   0.7451(289)       &   1.7263(697)       &   0.4189(277)     \\ 
 $\Sigma_c^{0}       $                &   -       &   0.6575(345)                 &   -      &   -0.2993(191)      &   -0.6575(345)       &   0.6575(345)       &   1.5656(783)       &   0.3656(319)     \\ 
 $\Xi_c^{\prime +}   $      &   0.3785(127)                 &   -        &   0.4513(75)      &   -0.3181(116)       &   0.3785(127)      &   -0.5252(136)       &   1.7837(434)       &   0.5131(183)     \\ 
 $\Xi_c^{\prime 0}   $                &   -       &   0.3379(131)        &   0.4581(75)      &   -0.3256(102)      &   -0.3379(131)      &   -0.3379(131)       &   1.7753(387)       &   0.4700(167)     \\ 
 $\Omega_c^0         $                &   -                 &   -       &   0.8662(111)       &   -0.3178(74)                 &   -      &   -1.7325(221)       &   1.8199(275)       &   0.5484(112)     \\ 
 $\Sigma_c^{*++}     $      &   1.2003(504)                 &   -                 &   -       &   0.9021(169)       &   1.2003(504)       &   1.2003(504)      &   -1.5050(596)       &   2.1022(578)     \\ 
 $\Sigma_c^{*+}      $      &   0.5690(290)       &   0.5381(307)                 &   -       &   0.9196(132)       &   0.0311(378)       &   1.1064(463)      &   -1.6484(489)       &   2.0253(524)     \\ 
 $\Sigma_c^{*0}      $                &   -       &   1.0579(566)                 &   -       &   0.9146(158)      &   -1.0579(566)       &   1.0579(566)      &   -1.6835(631)       &   1.9796(630)     \\ 
 $\Xi_c^{*+}         $      &   0.5821(210)                 &   -       &   0.6787(232)       &   0.9028(105)       &   0.5821(210)      &   -0.7672(321)      &   -1.4583(360)       &   2.1547(349)     \\ 
 $\Xi_c^{*0}         $                &   -       &   0.5478(244)       &   0.6378(136)        &   0.9127(99)      &   -0.5478(244)      &   -0.7213(325)      &   -1.5525(366)       &   2.1019(339)     \\ 
 $\Omega_c^{*0}      $                &   -                 &   -       &   1.3098(180)        &   0.9121(82)                 &   -      &   -2.6195(360)      &   -1.4260(217)       &   2.2227(233)     \\ 
 $\Xi_{cc}^{++}      $      &   -0.2020(84)                 &   -                 &   -        &   1.1992(87)       &   -0.2020(84)       &   -0.2020(84)      &   -3.7995(299)        &   1.0002(99)     \\ 
 $\Xi_{cc}^{+}       $                &   -       &   -0.1986(84)                 &   -        &   1.1924(83)        &   0.1986(84)       &   -0.1986(84)      &   -3.7729(282)       &   0.9954(102)     \\ 
 $\Omega_{cc}^+      $                &   -                 &   -       &   -0.2242(40)        &   1.1826(98)                 &   -        &   0.4484(79)      &   -3.7781(321)       &   0.9523(109)     \\ 
 $\Xi_{cc}^{*++}     $      &   0.5875(216)                 &   -                 &   -       &   1.7914(169)       &   0.5875(216)       &   0.5875(216)      &   -4.7909(451)       &   2.3794(266)     \\ 
 $\Xi_{cc}^{*+}      $                &   -       &   0.5303(236)                 &   -       &   1.8079(140)      &   -0.5303(236)       &   0.5303(236)      &   -4.8895(469)       &   2.3385(281)     \\ 
 $\Omega_{cc}^{*+}   $                &   -                 &   -        &   0.6425(82)       &   1.7929(115)                 &   -      &   -1.2851(164)      &   -4.7365(324)       &   2.4354(165)     \\ 
 $\Omega_{ccc}^{++}  $                &   -                 &   -                 &   -       &   2.6214(247)                 &   -                 &   -      &   -7.8641(741)       &   2.6214(247)     \\ 


==> tables/table_B35.tex <==
 $ N                 $     &   -0.2912(231)       &   0.8310(370)                 &   -                 &   -       &   1.1267(379)       &   0.5599(284)       &   0.5599(284)       &   0.5599(284)     \\ 
 $\Lambda            $      &   0.0107(108)      &   -0.0789(105)       &   0.7082(110)                 &   -       &   0.0894(157)      &   -1.4839(270)       &   0.6392(178)       &   0.6392(178)     \\ 
 $\Sigma^+           $      &   0.8149(401)                 &   -      &   -0.2651(178)                 &   -       &   0.8149(401)       &   1.3448(577)       &   0.5509(415)       &   0.5509(415)     \\ 
 $\Sigma^0           $      &   0.4304(197)       &   0.3303(154)      &   -0.2625(119)                 &   -       &   0.1008(247)       &   1.2849(362)       &   0.4976(264)       &   0.4976(264)     \\ 
 $\Sigma^-           $                &   -       &   0.7877(286)      &   -0.2853(133)                 &   -      &   -0.7877(286)       &   1.3569(419)       &   0.5037(296)       &   0.5037(296)     \\ 
 $\Xi^0              $     &   -0.2685(161)                 &   -       &   0.9299(177)                 &   -      &   -0.2685(161)      &   -2.1291(412)       &   0.6619(219)       &   0.6619(219)     \\ 
 $\Xi^-              $                &   -      &   -0.2550(106)       &   0.9194(176)                 &   -       &   0.2550(106)      &   -2.0972(339)       &   0.6673(144)       &   0.6673(144)     \\ 
 $\Delta^{++}        $     &   1.7005(1042)                 &   -                 &   -                 &   -      &   1.7005(1042)      &   1.7005(1042)      &   1.7005(1042)      &   1.7005(1042)     \\ 
 $\Delta^{+}         $      &   1.1725(925)       &   0.5305(594)                 &   -                 &   -       &   0.6386(978)      &   1.6967(1211)      &   1.6967(1211)      &   1.6967(1211)     \\ 
 $\Delta^{0}         $      &   0.5287(693)       &   1.0053(971)                 &   -                 &   -     &   -0.4807(1065)      &   1.5280(1306)      &   1.5280(1306)      &   1.5280(1306)     \\ 
 $\Delta^{-}         $                &   -      &   1.4401(1333)                 &   -                 &   -     &   -1.4401(1333)      &   1.4401(1333)      &   1.4401(1333)      &   1.4401(1333)     \\ 
 $\Sigma^{*+}        $      &   1.2863(638)                 &   -       &   0.6951(260)                 &   -       &   1.2863(638)      &   -0.1015(486)       &   1.9814(833)       &   1.9814(833)     \\ 
 $\Sigma^{*0}        $      &   0.5965(315)       &   0.5297(371)       &   0.6428(230)                 &   -       &   0.0655(445)      &   -0.1576(468)       &   1.7656(670)       &   1.7656(670)     \\ 
 $\Sigma^{*-}        $                &   -       &   1.0443(620)       &   0.6405(278)                 &   -      &   -1.0443(620)      &   -0.2318(717)       &   1.6813(737)       &   1.6813(737)     \\ 
 $\Xi^{*0}           $      &   0.6215(256)                 &   -       &   1.3622(366)                 &   -       &   0.6215(256)      &   -2.1007(606)       &   1.9839(563)       &   1.9839(563)     \\ 
 $\Xi^{*-}           $                &   -       &   0.5470(299)       &   1.3239(334)                 &   -      &   -0.5470(299)      &   -2.1012(648)       &   1.8727(503)       &   1.8727(503)     \\ 
 $\Omega^-           $                &   -                 &   -       &   2.0253(442)                 &   -                 &   -      &   -4.0506(885)       &   2.0253(442)       &   2.0253(442)     \\ 
 $\Lambda_c^+        $      &   -0.0036(64)       &   -0.0200(63)                 &   -        &   0.9204(76)        &   0.0167(87)       &   -0.0239(93)      &   -2.7845(262)       &   0.8994(107)     \\ 
 $\Xi_c^+            $      &   -0.0269(63)                 &   -       &   -0.0014(42)        &   0.9236(84)       &   -0.0269(63)      &   -0.0836(320)      &   -2.8017(224)       &   0.8904(143)     \\ 
 $\Xi_c^0            $                &   -       &   -0.0274(51)        &   0.0088(40)        &   0.9202(63)        &   0.0274(51)        &   0.0274(51)      &   -2.7799(198)        &   0.9043(90)     \\ 
 $\Sigma_c^{++}      $      &   0.7783(310)                 &   -                 &   -      &   -0.3170(178)       &   0.7783(310)       &   0.7783(310)       &   1.7316(674)       &   0.4623(323)     \\ 
 $\Sigma_c^{+}       $      &   0.3850(159)       &   0.3376(151)                 &   -      &   -0.3239(144)       &   0.0473(207)       &   0.7216(230)       &   1.6929(551)       &   0.3982(229)     \\ 
 $\Sigma_c^{0}       $                &   -       &   0.7114(280)                 &   -      &   -0.3137(178)      &   -0.7114(280)       &   0.7114(280)       &   1.6500(664)       &   0.4013(293)     \\ 
 $\Xi_c^{\prime +}   $      &   0.3740(125)                 &   -        &   0.4395(80)      &   -0.3156(111)       &   0.3740(125)      &   -0.5055(136)       &   1.7612(420)       &   0.4982(187)     \\ 
 $\Xi_c^{\prime 0}   $                &   -       &   0.3358(113)        &   0.4529(88)       &   -0.3142(94)      &   -0.3358(113)      &   -0.3358(113)       &   1.7303(363)       &   0.4744(158)     \\ 
 $\Omega_c^0         $                &   -                 &   -       &   0.8553(129)       &   -0.3158(77)                 &   -      &   -1.7106(258)       &   1.8031(298)       &   0.5398(128)     \\ 
 $\Sigma_c^{*++}     $      &   1.1494(530)                 &   -                 &   -       &   0.9055(177)       &   1.1494(530)       &   1.1494(530)      &   -1.5704(610)       &   2.0540(613)     \\ 
 $\Sigma_c^{*+}      $      &   0.5438(240)       &   0.4978(242)                 &   -       &   0.9033(142)       &   0.0449(321)       &   1.0402(358)      &   -1.6657(433)       &   1.9413(435)     \\ 
 $\Sigma_c^{*0}      $                &   -       &   0.9546(448)                 &   -       &   0.9182(170)      &   -0.9546(448)       &   0.9546(448)      &   -1.7894(577)       &   1.8706(522)     \\ 
 $\Xi_c^{*+}         $      &   0.5584(214)                 &   -       &   0.6271(156)       &   0.9034(135)       &   0.5584(214)      &   -0.6989(227)      &   -1.5276(387)       &   2.0868(422)     \\ 
 $\Xi_c^{*0}         $                &   -       &   0.5220(215)       &   0.6253(145)       &   0.9028(119)      &   -0.5220(215)      &   -0.7156(399)      &   -1.5625(322)       &   2.0488(369)     \\ 
 $\Omega_c^{*0}      $                &   -                 &   -       &   1.2827(234)        &   0.9027(99)                 &   -      &   -2.5654(467)      &   -1.4294(267)       &   2.1850(299)     \\ 
 $\Xi_{cc}^{++}      $      &   -0.2038(78)                 &   -                 &   -        &   1.2140(81)       &   -0.2038(78)       &   -0.2038(78)      &   -3.8456(268)       &   1.0103(102)     \\ 
 $\Xi_{cc}^{+}       $                &   -       &   -0.1932(74)                 &   -        &   1.2164(84)        &   0.1932(74)       &   -0.1932(74)      &   -3.8429(267)       &   1.0233(108)     \\ 
 $\Omega_{cc}^+      $                &   -                 &   -       &   -0.2202(42)        &   1.2013(73)                 &   -        &   0.4405(85)      &   -3.8246(236)        &   0.9809(80)     \\ 
 $\Xi_{cc}^{*++}     $      &   0.5535(196)                 &   -                 &   -       &   1.7688(223)       &   0.5535(196)       &   0.5535(196)      &   -4.7564(664)       &   2.3193(358)     \\ 
 $\Xi_{cc}^{*+}      $                &   -       &   0.5159(187)                 &   -       &   1.7653(202)      &   -0.5159(187)       &   0.5159(187)      &   -4.7794(611)       &   2.2834(331)     \\ 
 $\Omega_{cc}^{*+}   $                &   -                 &   -       &   0.6194(106)       &   1.7727(140)                 &   -      &   -1.2388(213)      &   -4.6994(393)       &   2.3926(204)     \\ 
 $\Omega_{ccc}^{++}  $                &   -                 &   -                 &   -       &   2.5916(268)                 &   -                 &   -      &   -7.7749(803)       &   2.5916(268)     \\ 


==> tables/table_B55.tex <==
  $ N                 $    &   -0.2888(157)       &   0.8773(255)                 &   -                 &   -       &   1.1300(277)       &   0.5813(236)       &   0.5813(236)       &   0.5813(236)     \\ 
  $\Lambda            $      &   0.0091(96)      &   -0.0755(107)        &   0.7088(97)                 &   -       &   0.0847(142)      &   -1.4820(230)       &   0.6426(186)       &   0.6426(186)     \\ 
  $\Sigma^+           $     &   0.8318(249)                 &   -      &   -0.2572(140)                 &   -       &   0.8318(249)       &   1.3460(347)       &   0.5733(302)       &   0.5733(302)     \\ 
  $\Sigma^0           $     &   0.4954(141)       &   0.3524(133)       &   -0.2691(98)                 &   -       &   0.1426(172)       &   1.3865(289)       &   0.5790(234)       &   0.5790(234)     \\ 
  $\Sigma^-           $               &   -       &   0.8524(203)      &   -0.2776(104)                 &   -      &   -0.8524(203)       &   1.4076(311)       &   0.5741(215)       &   0.5741(215)     \\ 
  $\Xi^0              $    &   -0.2513(117)                 &   -       &   0.9320(162)                 &   -      &   -0.2513(117)      &   -2.1163(346)       &   0.6804(201)       &   0.6804(201)     \\ 
  $\Xi^-              $               &   -      &   -0.2432(109)       &   0.9188(138)                 &   -       &   0.2432(109)      &   -2.0798(312)       &   0.6733(162)       &   0.6733(162)     \\ 
  $\Delta^{++}        $     &   1.6768(853)                 &   -                 &   -                 &   -       &   1.6768(853)       &   1.6768(853)       &   1.6768(853)       &   1.6768(853)     \\ 
  $\Delta^{+}         $     &   1.0967(635)       &   0.5780(403)                 &   -                 &   -       &   0.5224(640)       &   1.6725(856)       &   1.6725(856)       &   1.6725(856)     \\ 
  $\Delta^{0}         $     &   0.4864(554)       &   1.0760(598)                 &   -                 &   -      &   -0.5686(636)      &   1.4911(1397)      &   1.4911(1397)      &   1.4911(1397)     \\ 
  $\Delta^{-}         $               &   -      &   1.5902(1272)                 &   -                 &   -     &   -1.5902(1272)      &   1.5902(1272)      &   1.5902(1272)      &   1.5902(1272)     \\ 
  $\Sigma^{*+}        $     &   1.1499(559)                 &   -       &   0.6522(238)                 &   -       &   1.1499(559)      &   -0.1500(357)       &   1.8014(760)       &   1.8014(760)     \\ 
  $\Sigma^{*0}        $     &   0.5512(269)       &   0.5666(284)       &   0.6169(202)                 &   -      &   -0.0130(324)      &   -0.1139(322)       &   1.7275(613)       &   1.7275(613)     \\ 
  $\Sigma^{*-}        $               &   -       &   1.1160(486)       &   0.5624(427)                 &   -      &   -1.1160(486)      &   -0.0664(505)       &   1.6671(816)       &   1.6671(816)     \\ 
  $\Xi^{*0}           $     &   0.5752(243)                 &   -       &   1.2760(364)                 &   -       &   0.5752(243)      &   -1.9795(555)       &   1.8488(577)       &   1.8488(577)     \\ 
  $\Xi^{*-}           $               &   -       &   0.5713(231)       &   1.2244(400)                 &   -      &   -0.5713(231)      &   -1.8951(737)       &   1.8078(484)       &   1.8078(484)     \\ 
  $\Omega^-           $               &   -                 &   -       &   1.9079(439)                 &   -                 &   -      &   -3.8158(879)       &   1.9079(439)       &   1.9079(439)     \\ 
  $\Lambda_c^+        $     &   -0.0019(58)       &   -0.0208(55)                 &   -        &   0.9400(64)        &   0.0187(83)       &   -0.0232(76)      &   -2.8422(212)        &   0.9173(95)     \\ 
  $\Xi_c^+            $     &   -0.0135(49)                 &   -       &   -0.0031(37)        &   0.9369(65)       &   -0.0135(49)       &   -0.0076(55)      &   -2.8268(222)        &   0.9207(94)     \\ 
  $\Xi_c^0            $               &   -       &   -0.0260(41)        &   0.0067(41)        &   0.9350(57)        &   0.0260(41)        &   0.0260(41)      &   -2.8235(181)        &   0.9161(77)     \\ 
  $\Sigma_c^{++}      $     &   0.7627(215)                 &   -                 &   -      &   -0.3043(173)       &   0.7627(215)       &   0.7627(215)       &   1.6756(585)       &   0.4585(259)     \\ 
  $\Sigma_c^{+}       $     &   0.4035(118)       &   0.3616(122)                 &   -      &   -0.3055(142)       &   0.0409(162)       &   0.7653(176)       &   1.6818(501)       &   0.4604(196)     \\ 
  $\Sigma_c^{0}       $               &   -       &   0.7802(201)                 &   -      &   -0.3038(143)      &   -0.7802(201)       &   0.7802(201)       &   1.6914(498)       &   0.4765(230)     \\ 
  $\Xi_c^{\prime +}   $      &   0.3813(95)                 &   -        &   0.4319(69)      &   -0.3082(120)        &   0.3813(95)       &   -0.4836(90)       &   1.7374(406)       &   0.5047(185)     \\ 
  $\Xi_c^{\prime 0}   $               &   -       &   0.3610(100)        &   0.4473(69)       &   -0.3045(96)      &   -0.3610(100)      &   -0.3610(100)       &   1.7218(337)       &   0.5035(147)     \\ 
  $\Omega_c^0         $               &   -                 &   -       &   0.8562(120)       &   -0.3095(86)                 &   -      &   -1.7123(240)       &   1.7846(296)       &   0.5464(141)     \\ 
  $\Sigma_c^{*++}     $     &   1.1397(404)                 &   -                 &   -       &   0.9127(148)       &   1.1397(404)       &   1.1397(404)      &   -1.5975(448)       &   2.0520(490)     \\ 
  $\Sigma_c^{*+}      $     &   0.5652(207)       &   0.5490(194)                 &   -       &   0.9173(141)       &   0.0176(245)       &   1.1133(317)      &   -1.6356(403)       &   2.0292(399)     \\ 
  $\Sigma_c^{*0}      $               &   -       &   1.1582(369)                 &   -       &   0.9189(148)      &   -1.1582(369)       &   1.1582(369)      &   -1.6020(481)       &   2.0769(438)     \\ 
  $\Xi_c^{*+}         $     &   0.5756(169)                 &   -       &   0.6264(129)       &   0.9163(121)       &   0.5756(169)      &   -0.6761(166)      &   -1.5453(347)       &   2.1188(353)     \\ 
  $\Xi_c^{*0}         $               &   -       &   0.5683(178)       &   0.6328(134)       &   0.9227(120)      &   -0.5683(178)      &   -0.6976(257)      &   -1.5661(340)       &   2.1240(331)     \\ 
  $\Omega_c^{*0}      $               &   -                 &   -       &   1.2825(216)       &   0.9184(102)                 &   -      &   -2.5650(432)      &   -1.4711(267)       &   2.2008(283)     \\ 
  $\Xi_{cc}^{++}      $     &   -0.2108(70)                 &   -                 &   -        &   1.2350(72)       &   -0.2108(70)       &   -0.2108(70)      &   -3.9157(244)        &   1.0237(87)     \\ 
  $\Xi_{cc}^{+}       $               &   -       &   -0.2130(73)                 &   -        &   1.2355(75)        &   0.2130(73)       &   -0.2130(73)      &   -3.9191(257)        &   1.0224(88)     \\ 
  $\Omega_{cc}^+      $               &   -                 &   -       &   -0.2214(43)        &   1.2072(97)                 &   -        &   0.4429(86)      &   -3.8390(323)        &   0.9919(83)     \\ 
  $\Xi_{cc}^{*++}     $     &   0.5712(158)                 &   -                 &   -       &   1.8019(197)       &   0.5712(158)       &   0.5712(158)      &   -4.8453(477)       &   2.3698(308)     \\ 
  $\Xi_{cc}^{*+}      $               &   -       &   0.5712(185)                 &   -       &   1.8377(158)      &   -0.5712(185)       &   0.5712(185)      &   -4.9427(473)       &   2.4089(267)     \\ 
  $\Omega_{cc}^{*+}   $               &   -                 &   -       &   0.6395(102)       &   1.8175(135)                 &   -      &   -1.2791(204)      &   -4.8131(378)       &   2.4571(199)     \\ 
  $\Omega_{ccc}^{++}  $               &   -                 &   -                 &   -       &   2.6741(232)                 &   -                 &   -      &   -8.0222(695)       &   2.6741(232)     \\ 


==> tables/table_B75.tex <==
  $ N                 $    &   -0.2964(164)       &   0.8855(204)                 &   -                 &   -       &   1.1966(210)       &   0.5991(196)       &   0.5991(196)       &   0.5991(196)     \\ 
  $\Lambda            $      &   0.0196(86)       &   -0.0895(90)        &   0.7172(91)                 &   -       &   0.1090(113)      &   -1.5039(202)       &   0.6479(181)       &   0.6479(181)     \\ 
  $\Sigma^+           $     &   0.8740(257)                 &   -      &   -0.2677(103)                 &   -       &   0.8740(257)       &   1.4046(300)       &   0.6058(292)       &   0.6058(292)     \\ 
  $\Sigma^0           $     &   0.4972(125)       &   0.3762(113)       &   -0.2697(83)                 &   -       &   0.1209(148)       &   1.4104(233)       &   0.6040(213)       &   0.6040(213)     \\ 
  $\Sigma^-           $               &   -       &   0.8843(180)      &   -0.2930(106)                 &   -      &   -0.8843(180)       &   1.4693(301)       &   0.5911(193)       &   0.5911(193)     \\ 
  $\Xi^0              $    &   -0.2550(104)                 &   -       &   0.9314(170)                 &   -      &   -0.2550(104)      &   -2.1183(355)       &   0.6754(198)       &   0.6754(198)     \\ 
  $\Xi^-              $               &   -      &   -0.2800(115)       &   0.9352(127)                 &   -       &   0.2800(115)      &   -2.1459(268)       &   0.6515(224)       &   0.6515(224)     \\ 
  $\Delta^{++}        $     &   1.8348(711)                 &   -                 &   -                 &   -       &   1.8348(711)       &   1.8348(711)       &   1.8348(711)       &   1.8348(711)     \\ 
  $\Delta^{+}         $     &   1.1985(520)       &   0.5811(295)                 &   -                 &   -       &   0.6141(479)       &   1.7752(701)       &   1.7752(701)       &   1.7752(701)     \\ 
  $\Delta^{0}         $     &   0.5831(332)       &   1.1789(524)                 &   -                 &   -      &   -0.5960(490)       &   1.7598(726)       &   1.7598(726)       &   1.7598(726)     \\ 
  $\Delta^{-}         $               &   -       &   1.8142(869)                 &   -                 &   -      &   -1.8142(869)       &   1.8142(869)       &   1.8142(869)       &   1.8142(869)     \\ 
  $\Sigma^{*+}        $     &   1.2251(474)                 &   -       &   0.6560(209)                 &   -       &   1.2251(474)      &   -0.0888(221)       &   1.8819(666)       &   1.8819(666)     \\ 
  $\Sigma^{*0}        $     &   0.6041(228)       &   0.5865(244)       &   0.6503(192)                 &   -       &   0.0124(244)      &   -0.1115(248)       &   1.8376(573)       &   1.8376(573)     \\ 
  $\Sigma^{*-}        $               &   -       &   1.1787(451)       &   0.6464(235)                 &   -      &   -1.1787(451)      &   -0.1109(433)       &   1.8239(614)       &   1.8239(614)     \\ 
  $\Xi^{*0}           $     &   0.6071(213)                 &   -       &   1.3072(344)                 &   -       &   0.6071(213)      &   -2.0062(516)       &   1.9148(538)       &   1.9148(538)     \\ 
  $\Xi^{*-}           $               &   -       &   0.5896(224)       &   1.3017(335)                 &   -      &   -0.5896(224)      &   -2.0138(586)       &   1.8887(492)       &   1.8887(492)     \\ 
  $\Omega^-           $               &   -                 &   -       &   1.9599(458)                 &   -                 &   -      &   -3.9197(916)       &   1.9599(458)       &   1.9599(458)     \\ 
  $\Lambda_c^+        $      &   0.0025(46)       &   -0.0172(41)                 &   -        &   0.9356(58)        &   0.0193(55)       &   -0.0152(67)      &   -2.8220(184)        &   0.9212(91)     \\ 
  $\Xi_c^+            $     &   -0.0112(37)                 &   -        &   0.0028(80)        &   0.9305(56)       &   -0.0112(37)       &   -0.0015(44)      &   -2.8082(175)        &   0.9152(92)     \\ 
  $\Xi_c^0            $               &   -       &   -0.0211(34)        &   0.0067(34)        &   0.9338(52)        &   0.0211(34)        &   0.0211(34)      &   -2.8169(164)        &   0.9195(75)     \\ 
  $\Sigma_c^{++}      $     &   0.8291(210)                 &   -                 &   -      &   -0.3303(142)       &   0.8291(210)       &   0.8291(210)       &   1.8186(505)       &   0.4977(233)     \\ 
  $\Sigma_c^{+}       $     &   0.4138(101)        &   0.4078(99)                 &   -      &   -0.3159(119)       &   0.0065(115)       &   0.8220(165)       &   1.7696(417)       &   0.5059(188)     \\ 
  $\Sigma_c^{0}       $               &   -       &   0.8465(191)                 &   -      &   -0.3249(151)      &   -0.8465(191)       &   0.8465(191)       &   1.8209(534)       &   0.5221(210)     \\ 
  $\Xi_c^{\prime +}   $      &   0.4023(95)                 &   -        &   0.4398(75)      &   -0.3279(105)        &   0.4023(95)       &   -0.4779(81)       &   1.8250(374)       &   0.5139(186)     \\ 
  $\Xi_c^{\prime 0}   $               &   -        &   0.4004(89)        &   0.4466(77)       &   -0.3141(96)       &   -0.4004(89)       &   -0.4004(89)       &   1.7891(332)       &   0.5328(159)     \\ 
  $\Omega_c^0         $               &   -                 &   -       &   0.8610(133)       &   -0.3240(83)                 &   -      &   -1.7221(266)       &   1.8333(294)       &   0.5369(151)     \\ 
  $\Sigma_c^{*++}     $     &   1.2183(361)                 &   -                 &   -       &   0.9110(121)       &   1.2183(361)       &   1.2183(361)      &   -1.5192(416)       &   2.1278(419)     \\ 
  $\Sigma_c^{*+}      $     &   0.5838(174)       &   0.6184(166)                 &   -       &   0.9196(110)      &   -0.0355(176)       &   1.2036(292)      &   -1.5584(347)       &   2.1225(350)     \\ 
  $\Sigma_c^{*0}      $               &   -       &   1.1845(317)                 &   -       &   0.9179(121)      &   -1.1845(317)       &   1.1845(317)      &   -1.5698(387)       &   2.1026(378)     \\ 
  $\Xi_c^{*+}         $     &   0.5936(167)                 &   -       &   0.6428(127)       &   0.8849(185)       &   0.5936(167)      &   -0.6938(135)      &   -1.4802(331)       &   2.1403(336)     \\ 
  $\Xi_c^{*0}         $               &   -       &   0.6119(162)       &   0.6337(130)       &   0.9068(114)      &   -0.6119(162)      &   -0.6560(233)      &   -1.4897(296)       &   2.1573(301)     \\ 
  $\Omega_c^{*0}      $               &   -                 &   -       &   1.2893(226)       &   0.8920(157)                 &   -      &   -2.5787(452)      &   -1.4305(276)       &   2.1778(381)     \\ 
  $\Xi_{cc}^{++}      $     &   -0.1976(66)                 &   -                 &   -        &   1.2007(73)       &   -0.1976(66)       &   -0.1976(66)      &   -3.7987(249)        &   1.0034(80)     \\ 
  $\Xi_{cc}^{+}       $               &   -       &   -0.2066(57)                 &   -        &   1.2089(73)        &   0.2066(57)       &   -0.2066(57)      &   -3.8333(239)        &   1.0020(81)     \\ 
  $\Omega_{cc}^+      $               &   -                 &   -       &   -0.2144(48)       &   1.1850(111)                 &   -        &   0.4289(97)      &   -3.7647(366)        &   0.9789(86)     \\ 
  $\Xi_{cc}^{*++}     $     &   0.5844(148)                 &   -                 &   -       &   1.7662(223)       &   0.5844(148)       &   0.5844(148)      &   -4.7436(545)       &   2.3517(320)     \\ 
  $\Xi_{cc}^{*+}      $               &   -       &   0.5854(141)                 &   -       &   1.7628(240)      &   -0.5854(141)       &   0.5854(141)      &   -4.7033(730)       &   2.3437(347)     \\ 
  $\Omega_{cc}^{*+}   $               &   -                 &   -        &   0.6297(97)       &   1.7794(133)                 &   -      &   -1.2593(193)      &   -4.7093(382)       &   2.4090(185)     \\ 
  $\Omega_{ccc}^{++}  $               &   -                 &   -                 &   -       &   2.6153(222)                 &   -                 &   -      &   -7.8459(667)       &   2.6153(222)     \\ 


==> tables/table_D15.tex <==
 $ N                 $     &   -0.2802(280)       &   0.8078(402)                 &   -                 &   -       &   1.1392(347)       &   0.5034(385)       &   0.5034(385)       &   0.5034(385)     \\ 
 $\Lambda            $      &   0.0006(114)      &   -0.0776(124)       &   0.7152(102)                 &   -       &   0.0778(156)      &   -1.5051(287)       &   0.6394(199)       &   0.6394(199)     \\ 
 $\Sigma^+           $      &   0.7703(319)                 &   -      &   -0.2604(153)                 &   -       &   0.7703(319)       &   1.2889(435)       &   0.5089(357)       &   0.5089(357)     \\ 
 $\Sigma^0           $      &   0.4277(168)       &   0.3749(165)      &   -0.2680(108)                 &   -       &   0.0522(241)       &   1.3419(284)       &   0.5348(272)       &   0.5348(272)     \\ 
 $\Sigma^-           $                &   -       &   0.8104(281)      &   -0.2601(130)                 &   -      &   -0.8104(281)       &   1.3314(364)       &   0.5509(321)       &   0.5509(321)     \\ 
 $\Xi^0              $     &   -0.2373(122)                 &   -       &   0.9202(169)                 &   -      &   -0.2373(122)      &   -2.0932(269)       &   0.6873(190)       &   0.6873(190)     \\ 
 $\Xi^-              $                &   -      &   -0.2511(103)       &   0.9349(112)                 &   -       &   0.2511(103)      &   -2.1189(263)       &   0.6728(198)       &   0.6728(198)     \\ 
 $\Delta^{++}        $      &   1.8352(939)                 &   -                 &   -                 &   -       &   1.8352(939)       &   1.8352(939)       &   1.8352(939)       &   1.8352(939)     \\ 
 $\Delta^{+}         $      &   1.2418(897)      &   0.8800(1373)                 &   -                 &   -       &   0.5158(977)      &   1.9706(1115)      &   1.9706(1115)      &   1.9706(1115)     \\ 
 $\Delta^{0}         $      &   0.5975(557)       &   1.2404(811)                 &   -                 &   -      &   -0.6471(969)       &   1.8350(981)       &   1.8350(981)       &   1.8350(981)     \\ 
 $\Delta^{-}         $                &   -      &   1.7015(1416)                 &   -                 &   -     &   -1.7015(1416)      &   1.7015(1416)      &   1.7015(1416)      &   1.7015(1416)     \\ 
 $\Sigma^{*+}        $      &   1.1877(518)                 &   -       &   0.7009(206)                 &   -       &   1.1877(518)      &   -0.2100(435)       &   1.8897(659)       &   1.8897(659)     \\ 
 $\Sigma^{*0}        $      &   0.5961(310)       &   0.7125(528)       &   0.6946(189)                 &   -      &   -0.1361(682)      &   -0.1115(479)       &   1.9667(621)       &   1.9667(621)     \\ 
 $\Sigma^{*-}        $                &   -       &   1.2578(514)       &   0.6899(231)                 &   -      &   -1.2578(514)      &   -0.1206(611)       &   1.9470(609)       &   1.9470(609)     \\ 
 $\Xi^{*0}           $      &   0.5843(215)                 &   -       &   1.3652(271)                 &   -       &   0.5843(215)      &   -2.1469(462)       &   1.9472(427)       &   1.9472(427)     \\ 
 $\Xi^{*-}           $                &   -       &   0.6653(380)       &   1.3847(275)                 &   -      &   -0.6653(380)      &   -2.1210(534)       &   2.0341(437)       &   2.0341(437)     \\ 
 $\Omega^-           $                &   -                 &   -       &   2.0276(302)                 &   -                 &   -      &   -4.0552(604)       &   2.0276(302)       &   2.0276(302)     \\ 
 $\Lambda_c^+        $      &   -0.0116(57)       &   -0.0173(58)                 &   -        &   0.9010(95)        &   0.0059(74)       &   -0.0292(87)      &   -2.7483(267)        &   0.8844(89)     \\ 
 $\Xi_c^+            $      &   -0.0157(45)                 &   -       &   -0.0076(30)        &   0.9087(57)       &   -0.0157(45)       &   -0.0008(62)      &   -2.7484(196)        &   0.8884(92)     \\ 
 $\Xi_c^0            $                &   -       &   -0.0204(41)        &   0.0004(31)        &   0.8998(63)        &   0.0204(41)        &   0.0204(41)      &   -2.7299(164)        &   0.8790(98)     \\ 
 $\Sigma_c^{++}      $      &   0.7312(260)                 &   -                 &   -      &   -0.2987(151)       &   0.7312(260)       &   0.7312(260)       &   1.6286(575)       &   0.4347(266)     \\ 
 $\Sigma_c^{+}       $      &   0.3820(156)       &   0.3980(153)                 &   -      &   -0.3132(118)      &   -0.0160(203)       &   0.7803(233)       &   1.7186(454)       &   0.4676(242)     \\ 
 $\Sigma_c^{0}       $                &   -       &   0.7661(262)                 &   -      &   -0.2928(144)      &   -0.7661(262)       &   0.7661(262)       &   1.6447(511)       &   0.4755(299)     \\ 
 $\Xi_c^{\prime +}   $      &   0.3484(115)                 &   -        &   0.4443(59)       &   -0.3126(78)       &   0.3484(115)      &   -0.5363(122)       &   1.7338(307)       &   0.4817(152)     \\ 
 $\Xi_c^{\prime 0}   $                &   -       &   0.3747(122)        &   0.4532(66)       &   -0.3089(74)      &   -0.3747(122)      &   -0.3747(122)       &   1.7578(279)       &   0.5213(160)     \\ 
 $\Omega_c^0         $                &   -                 &   -       &   0.8424(153)       &   -0.3119(51)                 &   -      &   -1.6847(305)       &   1.7995(204)       &   0.5326(147)     \\ 
 $\Sigma_c^{*++}     $      &   1.1236(422)                 &   -                 &   -       &   0.9054(112)       &   1.1236(422)       &   1.1236(422)      &   -1.5909(484)       &   2.0279(458)     \\ 
 $\Sigma_c^{*+}      $      &   0.5694(276)       &   0.6126(281)                 &   -        &   0.9047(96)      &   -0.0458(341)       &   1.1804(442)      &   -1.5321(463)       &   2.0836(475)     \\ 
 $\Sigma_c^{*0}      $                &   -       &   1.1545(421)                 &   -       &   0.8970(103)      &   -1.1545(421)       &   1.1545(421)      &   -1.5334(497)       &   2.0503(444)     \\ 
 $\Xi_c^{*+}         $      &   0.5475(206)                 &   -       &   0.6478(112)        &   0.9071(78)       &   0.5475(206)      &   -0.7468(223)      &   -1.5231(313)       &   2.0998(306)     \\ 
 $\Xi_c^{*0}         $                &   -       &   0.5959(225)       &   0.6687(113)        &   0.9051(74)      &   -0.5959(225)      &   -0.7422(287)      &   -1.4493(295)       &   2.1701(303)     \\ 
 $\Omega_c^{*0}      $                &   -                 &   -       &   1.2544(293)       &   0.8895(102)                 &   -      &   -2.5088(586)      &   -1.3996(174)       &   2.1487(321)     \\ 
 $\Xi_{cc}^{++}      $      &   -0.1845(70)                 &   -                 &   -        &   1.1987(52)       &   -0.1845(70)       &   -0.1845(70)      &   -3.7803(183)        &   1.0134(78)     \\ 
 $\Xi_{cc}^{+}       $                &   -       &   -0.1887(67)                 &   -        &   1.1955(54)        &   0.1887(67)       &   -0.1887(67)      &   -3.7742(186)        &   1.0058(78)     \\ 
 $\Omega_{cc}^+      $                &   -                 &   -       &   -0.2143(36)        &   1.1779(59)                 &   -        &   0.4287(71)      &   -3.7443(196)        &   0.9681(51)     \\ 
 $\Xi_{cc}^{*++}     $      &   0.5411(210)                 &   -                 &   -       &   1.7824(135)       &   0.5411(210)       &   0.5411(210)      &   -4.8201(422)       &   2.2723(435)     \\ 
 $\Xi_{cc}^{*+}      $                &   -       &   0.5382(198)                 &   -       &   1.7789(149)      &   -0.5382(198)       &   0.5382(198)      &   -4.8079(458)       &   2.3166(252)     \\ 
 $\Omega_{cc}^{*+}   $                &   -                 &   -        &   0.6342(77)        &   1.7818(87)                 &   -      &   -1.2683(155)      &   -4.7122(242)       &   2.4147(136)     \\ 
 $\Omega_{ccc}^{++}  $                &   -                 &   -                 &   -       &   2.6068(159)                 &   -                 &   -      &   -7.8203(478)       &   2.6068(159)     \\ 

